High-dimensional Black-box Optimization Under Uncertainty

Optimizing expensive black-box systems with limited data is an extremely challenging problem. As a resolution, we present a new surrogate optimization approach by addressing two gaps in prior research -- unimportant input variables and inefficient treatment of uncertainty associated with the black-box output. We first design a new flexible non-interpolating parsimonious surrogate model using a partitioning-based multivariate adaptive regression splines approach, Tree Knot MARS (TK-MARS). The proposed model is specifically designed for optimization by capturing the structure of the function, bending at near-optimal locations, and is capable of screening unimportant input variables. Furthermore, we develop a novel replication approach called \emph{Smart-Replication}, to overcome the uncertainty associated with the black-box output. The Smart-Replication approach identifies promising input points to replicate and avoids unnecessary evaluations of other data points. Smart-Replication is agnostic to the choice of a surrogate and can adapt itself to an unknown noise level. Finally to demonstrate the effectiveness of our proposed approaches we consider different complex global optimization test functions from the surrogate optimization literature. The results indicate that TK-MARS outperforms original MARS within a surrogate optimization algorithm and successfully detects important variables. The results also show that although non-interpolating surrogates can mitigate uncertainty, replication is still beneficial for optimizing highly complex black-box functions. The robustness and the quality of the final optimum solution found through Smart-Replication are competitive with that using no replications in environments with low levels of noise and using a fixed number of replications in highly noisy environments.

==> anova.tex <==
We perform an ANOVA on an OA-designed experiments to test the hypothesis of variations caused by different factors. In ANOVA, the reference population is the first level of each factor.
From the results, Table~\ref{tab:norep-anova-oa}, it can be observed that statistically significant parameters are the fraction of important factors ($\mathit{fiv}$) and the noise level ($np$). 
From the results, Table~\ref{tab:norep-anova-oa}, it can be observed that statistically significant parameters are the fraction of important factors ($\mathit{fiv}$) and the noise level ($np$). 
This indicates that the deterministic approach can not handle the noise effect and has an important impact on the algorithm efficiency (MTFAUC).

\begin{table}[!tb]
\vspace{-3mm}
  \centering
  \caption{No-Replication ANOVA table}
  \begin{scriptsize}
    \begin{tabular}{|lcccccc|}
          & \multicolumn{1}{l}{Estimate} & \multicolumn{1}{l}{Std. Error} & \multicolumn{1}{l}{t value} & \multicolumn{1}{l}{$Pr(>|t|)$} &       &  \\
    \multicolumn{1}{|l|}{(Intercept)} & 0.0213 & 0.06535 & 0.326 & 0.745659 &       &  \\
    \multicolumn{1}{|l|}{fiv=0.75} & 0.12197 & 0.04773 & 2.556 & 0.013294 & *     &  \\
    \multicolumn{1}{|l|}{fiv=0.50} & 0.22659 & 0.04773 & 4.748 & 1.43E-05 & ***   &  \\
    \multicolumn{1}{|l|}{fiv=0.25} & 0.30299 & 0.04773 & 6.348 & 3.84E-08 & ***   &  \\
    \multicolumn{1}{|l|}{noise level=10\%} & 0.14558 & 0.04133 & 3.522 & 0.000851 & ***   &  \\
    \multicolumn{1}{|l|}{noise level=25\%} & 0.23302 & 0.04133 & 5.638 & 5.59E-07 & ***   &  \\
    \multicolumn{1}{|l|}{Rastrigin} & 0.33031 & 0.04133 & 7.991 & 7.10E-11 & ***   &  \\
    \multicolumn{1}{|l|}{Levy} & -0.02759 & 0.04133 & -0.667 & 0.507163 &       &  \\
    \multicolumn{1}{|l|}{dimension=20} & -0.06038 & 0.04133 & -1.461 & 0.149573 &       &  \\
    \multicolumn{1}{|l|}{dimension=30} & 0.01005 & 0.04133 & 0.243 & 0.808709 &       &  \\
    \multicolumn{1}{|l|}{poolSize=2(d+1)} & 0.01179 & 0.03375 & 0.35  & 0.728 &       &  \\
    \multicolumn{1}{|l|}{DOE=Sobol} & -0.02552 & 0.03375 & -0.756 & 0.452732 &       &  \\
    \multicolumn{1}{|l|}{EEPA distance=Cosine} & 0.01675 & 0.03375 & 0.496 & 0.62165 &       &  \\
    \multicolumn{1}{|l|}{EEPA number of candidates=6} & 0.0452 & 0.03375 & 1.339 & 0.185774 &       &  \\
    \multicolumn{1}{|l|}{model=TK-MARS} & -0.01327 & 0.03375 & -0.393 & 0.695633 &       &  \\
    \multicolumn{1}{|r|}{} &       &       &       &       &       &  \\
    Signif. Codes: & 0 ‘***’ & 0.001 ‘**’ & 0.01 ‘*’ & 0.05 ‘.’ & 0.1 ‘ ’ & 1 \\
    \end{tabular}%
    \end{scriptsize}
  \label{tab:norep-anova-oa}%
  \vspace{-3mm}
\end{table}%

Next, we consider the replication approach to mitigate the effect of noise. An analysis of variance is performed with MTFAUC as the response variable on the set of parameters shown in Table~\ref{tab:wrep-OA}. We consider two $\mathit{fixedrep}$ and $\mathit{smartrep}$ replication types with two distinct replication numbers $5$ and $10$. 
The replication number for $\mathit{fixedrep}$ is the fixed number of replications for each candidate points, however, for $\mathit{smartrep}$ it is the maximum number of replications.

The replication number for $\mathit{fixedrep}$ is the fixed number of replications for each candidate points, however, for $\mathit{smartrep}$ it is the maximum number of replications.

From Table~\ref{tab:wrep-anova-oa}, note that the noise parameter is not significant anymore, which indicates that replication helps to cancel out the noise effect. TK-MARS is margina-  lly significant. The Smart-Replication strategy is statistically better than Fixed-Replication, which is consistent with our expectation. Using smart replication saves function evaluations and and in a noisy scenario decreases the MTFAUC.

\begin{table}[!tb]
  \centering
  \caption{Replication ANOVA table}
    \begin{scriptsize}
    \begin{tabular}{|lcccccc|}
    \multicolumn{1}{|r|}{} & \multicolumn{1}{l}{Estimate} & \multicolumn{1}{l}{Std. Error} & \multicolumn{1}{l}{t value} & \multicolumn{1}{l}{$Pr(>|t|)$} &       &  \\
    \multicolumn{1}{|l|}{(Intercept)} & \multicolumn{1}{r}{0.250806} & \multicolumn{1}{r}{0.086891} & \multicolumn{1}{r}{2.886} & \multicolumn{1}{r}{0.005626} & \multicolumn{1}{l}{**} &  \\
    \multicolumn{1}{|l|}{fiv=0.75} & \multicolumn{1}{r}{0.07965} & \multicolumn{1}{r}{0.056382} & \multicolumn{1}{r}{1.413} & \multicolumn{1}{r}{0.163596} &       &  \\
    \multicolumn{1}{|l|}{fiv=0.50} & \multicolumn{1}{r}{0.207822} & \multicolumn{1}{r}{0.056382} & \multicolumn{1}{r}{3.686} & \multicolumn{1}{r}{0.000537} & \multicolumn{1}{l}{***} &  \\
    \multicolumn{1}{|l|}{fiv=0.25} & \multicolumn{1}{r}{0.132775} & \multicolumn{1}{r}{0.056382} & \multicolumn{1}{r}{2.355} & \multicolumn{1}{r}{0.022263} & \multicolumn{1}{l}{*} &  \\
    \multicolumn{1}{|l|}{model=TK-MARS} & \multicolumn{1}{r}{0.113446} & \multicolumn{1}{r}{0.048828} & \multicolumn{1}{r}{2.323} & \multicolumn{1}{r}{0.024028} & \multicolumn{1}{l}{*} &  \\
    \multicolumn{1}{|l|}{noise level=10\%} & \multicolumn{1}{r}{0.004939} & \multicolumn{1}{r}{0.048828} & \multicolumn{1}{r}{0.101} & \multicolumn{1}{r}{0.91982} &       &  \\
    \multicolumn{1}{|l|}{noise level=25\%} & \multicolumn{1}{r}{0.009702} & \multicolumn{1}{r}{0.048828} & \multicolumn{1}{r}{0.199} & \multicolumn{1}{r}{0.843259} &       &  \\
    \multicolumn{1}{|l|}{smart\_rep} & \multicolumn{1}{r}{-0.09262} & \multicolumn{1}{r}{0.039868} & \multicolumn{1}{r}{-2.323} & \multicolumn{1}{r}{0.02404} & \multicolumn{1}{l}{*} &  \\
    \multicolumn{1}{|l|}{Rastrigin} & \multicolumn{1}{r}{0.344011} & \multicolumn{1}{r}{0.048828} & \multicolumn{1}{r}{7.045} & \multicolumn{1}{r}{3.81E-09} & \multicolumn{1}{l}{***} &  \\
    \multicolumn{1}{|l|}{Levy} & \multicolumn{1}{r}{0.045359} & \multicolumn{1}{r}{0.048828} & \multicolumn{1}{r}{0.929} & \multicolumn{1}{r}{0.357128} &       &  \\
    \multicolumn{1}{|l|}{dimension=20} & \multicolumn{1}{r}{0.073677} & \multicolumn{1}{r}{0.048828} & \multicolumn{1}{r}{1.509} & \multicolumn{1}{r}{0.137262} &       &  \\
    \multicolumn{1}{|l|}{dimension=30} & \multicolumn{1}{r}{0.051091} & \multicolumn{1}{r}{0.048828} & \multicolumn{1}{r}{1.046} & \multicolumn{1}{r}{0.300151} &       &  \\
    \multicolumn{1}{|l|}{Replication=10} & \multicolumn{1}{r}{0.146338} & \multicolumn{1}{r}{0.048828} & \multicolumn{1}{r}{2.997} & \multicolumn{1}{r}{0.004142} & \multicolumn{1}{l}{**} &  \\
    \multicolumn{1}{|l|}{poolSize=2(d+1)} & \multicolumn{1}{r}{0.016954} & \multicolumn{1}{r}{0.039868} & \multicolumn{1}{r}{0.425} & \multicolumn{1}{r}{0.67238} &       &  \\
    \multicolumn{1}{|l|}{DOE=Sobol} & \multicolumn{1}{r}{-0.00669} & \multicolumn{1}{r}{0.039868} & \multicolumn{1}{r}{-0.168} & \multicolumn{1}{r}{0.867332} &       &  \\
    \multicolumn{1}{|l|}{EEPA distance=Cosine} & \multicolumn{1}{r}{-0.01711} & \multicolumn{1}{r}{0.039868} & \multicolumn{1}{r}{-0.429} & \multicolumn{1}{r}{0.669465} &       &  \\
    \multicolumn{1}{|l|}{EEPA number of candidates=6} & \multicolumn{1}{r}{-0.02138} & \multicolumn{1}{r}{0.039868} & \multicolumn{1}{r}{-0.536} & \multicolumn{1}{r}{0.594059} &       &  \\
    \multicolumn{1}{|r|}{} &       &       &       &       &       &  \\
    Signif. Codes: & 0 ‘***’ & 0.001 ‘**’ & 0.01 ‘*’ & 0.05 ‘.’ & 0.1 ‘ ’ & 1 \\
    \end{tabular}%
    \end{scriptsize}
  \label{tab:wrep-anova-oa}%
\end{table}%
Looking at the ANOVA Tables~\ref{tab:norep-anova-oa} and~\ref{tab:wrep-anova-oa}, we drop the unimportant parameters to explore MTFAUC variation caused by important parameters and fixed them to the significant level identified by ANOVA.
Dimension=30, initial pool size=d+1, DOE method=LHD, EEPA distance=Euclidean, and EEPA number of candidate points is fixed to 3. We perform two separate full factorial designs considering the significant parameters; one for TK-MARS and one for RBF.
